SIM1: Physics-Aligned Simulator as Zero-Shot Data Scaler in Deformable Worlds

Robotic manipulation with deformable objects represents a data-intensive regime in embodied learning, where shape, contact, and topology co-evolve in ways that far exceed the variability of rigids. Although simulation promises relief from the cost of real-world data acquisition, prevailing sim-to-real pipelines remain rooted in rigid-body abstractions, producing mismatched geometry, fragile soft dynamics, and motion primitives poorly suited for cloth interaction. We posit that simulation fails not for being synthetic, but for being ungrounded. To address this, we introduce SIM1, a physics-aligned real-to-sim-to-real data engine that grounds simulation in the physical world. Given limited demonstrations, the system digitizes scenes into metric-consistent twins, calibrates deformable dynamics through elastic modeling, and expands behaviors via diffusion-based trajectory generation with quality filtering. This pipeline transforms sparse observations into scaled synthetic supervision with near-demonstration fidelity. Experiments show that policies trained on purely synthetic data achieve parity with real-data baselines at a 1:15 equivalence ratio, while delivering 90% zero-shot success and 50% generalization gains in real-world deployment. These results validate physics-aligned simulation as scalable supervision for deformable manipulation and a practical pathway for data-efficient policy learning.

==> sections/background.tex <==





\section{Background}
\label{sec:background}
The belief graph in our work is closely related to symbolic world representations.
\vspace{-1em}
\paragraph{World states.}  In classical AI, researchers use symbolic representations to describe the world state~\citep{McCHay69, minsky1974framework, minsky1988society, pasula2007learning, kaelbling2011hierarchical}. For example, in the blocks world~\citep{ginsberg1988reasoning, gupta1992complexity, alkhazraji-et-al-zenodo2020}, a state can be $$is\_block(a) \wedge is\_red(a) \wedge on\_table(a) \wedge is\_block(b) \wedge is\_blue(b) \wedge on(b, a),$$ describing that there are a red block and a blue block, referred to as $a$ and $b$, block $a$ is on a table, and block $b$ is on $a$. Such world states must include \textbf{entities} (e.g., $a$ and $b$), their \textbf{attributes} (e.g., position $on\_table$, characteristics $is\_block$) and \textbf{relations} (e.g., $on(b, a)$) which are critical for enabling a robot to know and act in the world.

In linguistics, \cite{davidson2001theories,davidson2001logical,davidson1967truth} introduce logic-based formalisms of meanings of sentences. The semantics of a sentence is decomposed to a set of atomic propositions, such that no propositions can be added or removed from the set to represent the meaning of the sentence. \citep{cho2023davidsonian} propose Davidsonian Scene Graph (DSG) which represent an image description as a set of atomic propositions (and corresponding questions about each proposition) to evaluate T2I alignment. %



We borrow the same concept as symbolic world representations and scene graphs, except that the agent needs to represent an imaginary world. The image generation problem can be viewed as taking a picture of the imaginary world. The world state should include all entities that are in the picture, together with their attributes and relations.


\vspace{-1em}
\paragraph{Belief states.} Term ``belief state''~\citep{nilsson1986probabilistic, kaelbling1998planning} has been used to describe a distribution over states. %
E.g., for block $a$, we might have $p(on\_table(a)) = 0.5$ and $p(\neg on\_table(a)) = 0.5$, which means the agent is unsure whether the block is on a table. To represent the T2I agent's belief on which image to generate, we need to consider the distribution over all possible ``worlds'' in which the picture can be taken. This distribution can be described by the probabilities that an entity appears in the picture, an attribute gets assigned a certain value, etc.

A core difference between our belief graphs and classic belief states is that belief graphs do not need pre-defined  predicates (e.g., $on(b, a)$), but instead automatically produce useful predicates using LLMs. This makes belief graphs much more generalizable across domains. More details in \S\ref{app:novelty}.

